Fluency-Guided Cross-Lingual Image Captioning

Image captioning has so far been explored mostly in English, as most available datasets are in this language. However, the application of image captioning should not be restricted by language. Only few studies have been conducted for image captioning in a cross-lingual setting. Different from these works that manually build a dataset for a target language, we aim to learn a cross-lingual captioning model fully from machine-translated sentences. To conquer the lack of fluency in the translated sentences, we propose in this paper a fluency-guided learning framework. The framework comprises a module to automatically estimate the fluency of the sentences and another module to utilize the estimated fluency scores to effectively train an image captioning model for the target language. As experiments on two bilingual (English-Chinese) datasets show, our approach improves both fluency and relevance of the generated captions in Chinese, but without using any manually written sentences from the target language.

==> dataset.tex <==

\subsection{Image captioning dataset}

To study cross-lingual image captioning, a prelimary need is a comparable corpus.

While previous works created this kind of dataset by mannually translating English captions or independently collecting new sentences in diffenrent languages using crowdsourcing, costing enormous amount of efforts, we extend the dataset by translating all English captions using machine translation and mannually translating only a small subset of the corpus.

Flickr8k-CN \cite{icmr2016} is a bilingual dataset for image captioning, which extends Flickr8k \cite{flickr8k} in two ways, by automatically translating the exsited English captions and independently collecting Chinese captions using crowdsourcing. Human translation of the English sentences in the test set are also provided.

Following \cite{icmr2016}, we further extend the Flickr30k \cite{flickr30k} dataset to a bilingual version?. 
%Collecting multilingual corpus by crowdsourcing tends? to get more reliable / cultural relevant captions. However it takes enumerous time and resources to build such datasets, and it is hard to extend to bigger dataset. We argue that it is eaiser to get more/ bigger multilingual data using machine translation.
%In this work, we further extend the flickr30k \cite{flickr30k} dataset to a multi-lingual dataset. 
The Flickr30k dataset consists of 158,915 crowd-sourced captions describing 31,783 images which are sourced from online photo-sharing websites. We use the same split as in \cite{iclr15-ma-mrnn}, which contains 145,000 training, 5,000 validation and 5,000 test descriptions. 
We applied machine translation \footnote{\url{http://fanyi.baidu.com}} to get Chinese sentences from training and validation sets and mannually translated the test set of the flickr30k into Chinese. The mannual translations were collected from Chinese colleage students who are fluent in English (passing the national College English Test 6). Translators were shown an English sentence as well as the image that was described in order to avoid ambiguity. For instance, football can be translated into \graybg{足球}(soccer) and \graybg{橄榄球}(American football) in Chinese.


\begin{table} [h!]
\renewcommand{\arraystretch}{1.2}
\caption{Dataset statistic}
\label{tab:caption_data_stat}
%
\centering
 \scalebox{0.9}{
\begin{tabular}{@{}p{2cm} l r r r rr r r@{}}
\toprule
&& \multicolumn{3}{c}{Flickr8k} && \multicolumn{3}{c}{Flickr30k} \\
\cmidrule{3-5} \cmidrule{7-9}
&& train & val & test && train & val & test \\
\cmidrule{1-9}
images  && 6,000  & 1,000 & 1,000 && 29,783 & 1,000 &1,000\\
\cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9}
\specialcell{English \\ sentences}  && 30,000  & 5,000 & 5,000 && 148,915 & 5,000 &5,000\\
\cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9}
machine translated sentences  && 30,000  & 5,000 & 5,000 && 148,915 & 5,000 &5,000\\
\cmidrule{1-1} \cmidrule{3-5} \cmidrule{7-9}
mannually translated  && -  & - & 5,000 && - & - &5,000\\

\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}


We compare our strtegies on the above two bilingual dataset, Flickr8k-CN and Flickr30k-CN, using the human translated captions as ground truth.



\subsection{Machine translated sentences evaluation dataset}

In order to train the sentence quality classification model, we collected 6,593 human labeled machine translated Chinese sentences. 
Although it is easy to obtain extra plain Chinese text data, we find that sentences in most other available text data (\eg news, wiki, SNS) do not share similar sentence struture or vocabulary with the captioning corpus therefore not suitable for this task. So we do not utilize this kind of text data.

Specifically, we first randomly chose 2,000, 2,000, and 4000 English captions from Flickr8k\cite{flickr8k}, Flickr30\cite{flickr8k} and MSCOCO\cite{mscoco} respectively, and translated them to Chinese sentences. Then we recruited a local crowdsourcing service to annotate these 8,000 sentences, asking annotators to answer the question of \textit{Do you think the sentence is fluent? (no obvious grammatical problems, in line with language habits of Chinese)} with a given machine translated Chinese sentence. 
To avoid the collected answers being too messy, three optional answers are provided, \ie \textit{fluent}, \textit{not fluent} and \textit{difficult to judge}. We hired five male and three female Chinese postgraduates, and divided them into four groups. Each group had two annotator. Everyone were asked to annotate 2,000 sentences, and annotators in the same group were asked to annotate same sentences. In order to ensure the quality of labeled sentences, we only keep the sentences annotated with the same answer by two distinct annotators and discard sentence annotated with answer of \textit{difficult to judge}. Finally, we obtain 6,593 labeled sentences, and randomly separate them into
4,593/1,000/1,000 for train/val/test splits, respectively. The number of fluent and not fluent sentences are summarized in Table \ref{tab:data_statistics}. The proportion of fluent sentences is about 30\% overall, which indicates the current machine translation system is far from perfect.


\begin{table} [h!]
\renewcommand{\arraystretch}{1.2}
\caption{The number of fluent and not fluent sentences in each split of the collected dataset. The low proportion of fluent sentences indicates the current machine translation system is far from perfect.}
\label{tab:data_statistics}
%
\centering
 \scalebox{0.99}{
\begin{tabular}{@{}l rrr@{}}
\toprule
%
   & \textbf{train} & \textbf{val} & \textbf{test}  \\
\cmidrule{1-4}
\# Fluent           & 1,240  & 291 & 294 \\
\# Not-fluent       & 3,353  & 709 & 706 \\
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}

% We randomly pick 8,000 baidu translated sentences to build a sentence-fluency dataset, where 2k sentences are from flickr8k\cite{flickr8k}, 4k sentences are from mscoco2014train, and 2k sentences are from mscoco2014val. 
% We hired eight native Chinese speakers/colleage students to annotate the fluency of the sentences. Each sentence is annotated by two different people. The annotators were shown one sentence each time and being asked that \"Do you consider this sentence fluent(comforming to the grammatical rules and the language habits of Chinese)?\". The candidate answers are \"Fluent\", \"Not fluent\" and \"Not sure\". Only sentences that are annotated as \"fluent\" by both annotators or \"not fluent\" by both annotators are kept in the final dataset. The other sentences are discarded. The resulting dataset consists of 6,593 sentences. We split the dataset into three splits, 

\subsection{Preprocessing }
Unlike western languages, many east Asian languages including Chinese are written without explicit word delimiters. Therefore, word segmentation is usually considered as a preliminary step for processing these languages.
We do the Chinese text segmentation through a service provided by bosonnlp \footnote{\url{https://github.com/bosondata/bosonnlp.py}}, a cloud based platform providing rich Chinese natural language processing service. We also generate the POS tags of Chinese sentences for sentence readability classifier by employing this service.

Moreover, it has been recognized that different NLP applications have different needs for word segmentation \cite{chang2008optimizing} .
Most Chinese NLP tasks could be expected to benefit by word segmentation because Chinese words can be composed of multiple characters whose meanings differ when presented individually(e.g. ...). However we consider character-based sequence model worth trying because sentences in image captioning task are rather simple and structured.


==> lstm_cl.tex <==
%=====================================================================================
%\section{Experiments}
%=====================================================================================

%\textbf{Implementation Details}.
% We employ Jieba\footnote{\url{https://github.com/fxsjy/jieba/}}, an open-source software for Chinese text segmentation and genrating POS tags of sentences. 
%For four individual models, we set the dimension of word embeddings to be 512, and size of LSTM to be 512. We replace words and POS tags that occurring less than two times in the training set with a special `UNK` token.
% Words and POS tags that occurring at least two times in the training set are kept, while other words and POS tags are replaced by a special `UNK` token.

%Unlike an English sentence that has spaces as explicit word boundary markers, a Chinese sentence lacks such markers. In order to tokenize a Chinese sentence into a list of meaningful words, we employ Jieba\footnote{\url{https://github.com/fxsjy/jieba/}}, an open-source software for Chinese text segmentation. We also use Jieba to generate the POS tags of sentences. We set the dimension of word embeddings to be 512, and size of LSTM to be 512 in our implementation.
% We only keep words and pos tags occurring at least tow times and in the training set , replacing discarded words and pos tags as a special <UNK> token.


% \textbf{Evaluation criteria}.
% precision, recall
% We report precision and recall which are widely used to evaluate classification model. Since we aim to better utilize sentences predicted to be fluent, we focus our discussion on the performance of the fluent class.
%As we only use sentences predicted to be fluent, we focus on the performance of the fluent class and ignore the not fluent one.
\textbf{Fluency dataset}

In order to train the sentence fluency classification model, we collected 6,594 human labeled machine translated Chinese sentences from image captioning corpus.
Although it is easy to obtain extra plain Chinese text data, we find that sentences in most other available text data (\eg news, wiki, SNS) do not share similar sentence struture or vocabulary with the captioning corpus therefore not suitable for this task. So we do not utilize this kind of text data.

Specifically, we first randomly chose 2,000, 2,000, and 4000 English captions from Flickr8k\cite{flickr8k}, Flickr30\cite{flickr8k} and MSCOCO\cite{mscoco} respectively, and translated them to Chinese sentences. Then we recruited a local crowdsourcing service to annotate these 8,000 sentences, asking annotators to answer the question of \textit{Do you think the sentence is fluent? (no obvious grammatical problems, in line with language habits of Chinese)} with a given machine translated Chinese sentence.
% To avoid the collected answers being too messy, t
Three optional answers are provided, \ie \textit{fluent}, \textit{not fluent} and \textit{difficult to judge}. We hired five male and three female Chinese postgraduates, and divided them into four groups. Each group had two annotator. Everyone were asked to annotate 2,000 sentences, and annotators in the same group were asked to annotate same sentences. In order to ensure the quality of labeled sentences, we only keep the sentences annotated with the same answer by two distinct annotators and discard sentence annotated with answer of \textit{difficult to judge}. Finally, we obtain 6,594 labeled sentences, and randomly separate them into
4,594/1,000/1,000 for train/val/test splits, respectively. The number of fluent and not fluent sentences are summarized in Table \ref{tab:data_statistics}. The proportion of fluent sentences is about 30\% overall, which indicates the current machine translation system is far from perfect.


\begin{table} [tb!]
\renewcommand{\arraystretch}{1.2}
\caption{The number of fluent and not fluent sentences in each split of the collected dataset. The low proportion of fluent sentences indicates the current machine translation system is far from perfect.}
\label{tab:data_statistics}
%
\centering
 \scalebox{0.99}{
\begin{tabular}{@{}l rrr@{}}
\toprule
%
   & \textbf{train} & \textbf{val} & \textbf{test}  \\
\cmidrule{1-4}
\# Fluent           & 1,240  & 291 & 294 \\
\# Not-fluent       & 3,353  & 709 & 706 \\
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}


\textbf{Results}.
% All the models are noticeably better than the random result. 
We present the recall and precision of the fluency model.
Since we attempt to better utilize sentences predicted to be fluent, and sentences that predicted to be not fluent can be utilized applying some strategies, we focus more on the precision of the model.
Table \ref{tab:class_perf} shows the performance of different models on our collected dataset. 
Since we have observed that longer sentences are translated with less fluency, we also present the performance of a length-based model as a baseline. Sentences with length longer than the average length of fluent sentences in the training set are predicted to be not fluent. Otherwise, they are predicted to be fluent.
Both two models based on machine translated Chinese sentences, \ie lstm(words$_{zh}$) and lstm(POS$_{zh}$), outperform its counterparts based on English sentences. This can be expected as we aim to predict the fluency of machine translated Chinese sentences. 
LSTM models perform better on precision than length-based model. Although we can get precision improvement using shorter length threshold, we argue that shorter sentences cannot provide @@@ information.

%Although t
The recall of fusing four individual models gets worse, but it gains precision improvement. As we use all sentences predicted to be fluent to train image captioning models, precision is more crucial. Hence, we utilize the results of average fusion for later training image captioning models.



\begin{table} [tb!]
\renewcommand{\arraystretch}{1.2}
\caption{Classification performance of the fluent class. Average fusion indicates late average fusion over predictions of four individual models.}
\label{tab:class_perf}
%
\centering
 \scalebox{0.99}{
\begin{tabular}{@{}l rrrr@{}}
\toprule
%
\textbf{Model}  && \textbf{Recall} & \textbf{Precision}  \\
\cmidrule{1-1} \cmidrule{3-4}
Random           && 0.500  & 0.294  \\ 
Length-based	 && 0.493  & 0.453  \\ [3pt]
lstm(words$_{zh}$)      && 0.503  &   0.617    \\
lstm(POS$_{zh}$)        && 0.449  &   0.626    \\
lstm(words$_{en}$)      && 0.371  &   0.580    \\
lstm(POS$_{en}$)        && 0.211  &   0.580    \\ [3pt]
Average fusion          && 0.340  &   0.800    \\
\bottomrule
\end{tabular}
 }% end of scalebox
\end{table}







% \begin{table} [h!]
% \renewcommand{\arraystretch}{1.2}
% \caption{Performance of classification models on the fluent sentences. lstm(words) is our classification model with original words as input, and lstm(POS tags) indicates the model with POS tags as input. }
% \label{tab:class_perf}
% %
% \centering
%  \scalebox{0.99}{
% \begin{tabular}{@{}l rr@{}}
% \toprule
% %
% \textbf{Model}   &&  \textbf{F1-score}  \\
% \cmidrule{1-1} \cmidrule{3-3}
% Random            && 0.370  \\ [3pt]
% lstm(words)       && 0.548  \\
% lstm(POS tags)    && 0.506  \\
% Average fusion    && 0.558  \\
% \bottomrule
% \end{tabular}
%  }% end of scalebox
% \end{table}


